Observation of associated production of a $Z$ boson with a $D$ meson in the~forward region

A search for associated production of a $Z$ boson with an open charm meson is presented using a data sample, corresponding to an integrated luminosity of $1.0\,\mathrm{fb}^{-`}$ of proton--proton collisions at a centre-of-mass energy of 7\,TeV, collected by the LHCb experiment. %% Seven candidate events for associated production of a $Z$ boson with a $D^0$ meson and four candidate events for a $Z$ boson with a $D^+$ meson are observed with a combined significance of 5.1standard deviations. The production cross-sections in the forward region are measured to be $$\sigma_{Z\rightarrow\mu^+\mu^-\!,D^0} = 2.50\pm1.12\pm0.22pb$$ $$\sigma_{Z\rightarrow\mu^+\mu^-\!,D^+} = 0.44\pm0.23\pm0.03pb,$$ where the first uncertainty is statistical and the second systematic.

==> LHCb_HD_comma_separated_author_2013-11-01.tex <==
LHCb collaboration:
R. Aaij, 
B. Adeva, 
M. Adinolfi, 
A. Affolder, 
Z. Ajaltouni, 
J. Albrecht, 
F. Alessio, 
M. Alexander, 
S. Ali, 
G. Alkhazov, 
P. Alvarez Cartelle, 
A.A. Alves Jr, 
S. Amato, 
S. Amerio, 
Y. Amhis, 
L. Anderlini, 
J. Anderson, 
R. Andreassen, 
M. Andreotti, 
J.E. Andrews, 
R.B. Appleby, 
O. Aquines Gutierrez, 
F. Archilli, 
A. Artamonov, 
M. Artuso, 
E. Aslanides, 
G. Auriemma, 
M. Baalouch, 
S. Bachmann, 
J.J. Back, 
A. Badalov, 
V. Balagura, 
W. Baldini, 
R.J. Barlow, 
C. Barschel, 
S. Barsuk, 
W. Barter, 
V. Batozskaya, 
Th. Bauer, 
A. Bay, 
J. Beddow, 
F. Bedeschi, 
I. Bediaga, 
S. Belogurov, 
K. Belous, 
I. Belyaev, 
E. Ben-Haim, 
G. Bencivenni, 
S. Benson, 
J. Benton, 
A. Berezhnoy, 
R. Bernet, 
M.-O. Bettler, 
M. van Beuzekom, 
A. Bien, 
S. Bifani, 
T. Bird, 
A. Bizzeti, 
P.M. Bj\o rnstad, 
T. Blake, 
F. Blanc, 
J. Blouw, 
S. Blusk, 
V. Bocci, 
A. Bondar, 
N. Bondar, 
W. Bonivento, 
S. Borghi, 
A. Borgia, 
M. Borsato, 
T.J.V. Bowcock, 
E. Bowen, 
C. Bozzi, 
T. Brambach, 
J. van den Brand, 
J. Bressieux, 
D. Brett, 
M. Britsch, 
T. Britton, 
N.H. Brook, 
H. Brown, 
A. Bursche, 
G. Busetto, 
J. Buytaert, 
S. Cadeddu, 
R. Calabrese, 
O. Callot, 
M. Calvi, 
M. Calvo Gomez, 
A. Camboni, 
P. Campana, 
D. Campora Perez, 
A. Carbone, 
G. Carboni, 
R. Cardinale, 
A. Cardini, 
H. Carranza-Mejia, 
L. Carson, 
K. Carvalho Akiba, 
G. Casse, 
L. Castillo Garcia, 
M. Cattaneo, 
Ch. Cauet, 
R. Cenci, 
M. Charles, 
Ph. Charpentier, 
S.-F. Cheung, 
N. Chiapolini, 
M. Chrzaszcz, 
K. Ciba, 
X. Cid Vidal, 
G. Ciezarek, 
P.E.L. Clarke, 
M. Clemencic, 
H.V. Cliff, 
J. Closier, 
C. Coca, 
V. Coco, 
J. Cogan, 
E. Cogneras, 
P. Collins, 
A. Comerma-Montells, 
A. Contu, 
A. Cook, 
M. Coombes, 
S. Coquereau, 
G. Corti, 
B. Couturier, 
G.A. Cowan, 
D.C. Craik, 
M. Cruz Torres, 
S. Cunliffe, 
R. Currie, 
C. D'Ambrosio, 
J. Dalseno, 
P. David, 
P.N.Y. David, 
A. Davis, 
I. De Bonis, 
K. De Bruyn, 
S. De Capua, 
M. De Cian, 
J.M. De Miranda, 
L. De Paula, 
W. De Silva, 
P. De Simone, 
D. Decamp, 
M. Deckenhoff, 
L. Del Buono, 
N. D\'{e}l\'{e}age, 
D. Derkach, 
O. Deschamps, 
F. Dettori, 
A. Di Canto, 
H. Dijkstra, 
S. Donleavy, 
F. Dordei, 
M. Dorigo, 
P. Dorosz, 
A. Dosil Su\'{a}rez, 
D. Dossett, 
A. Dovbnya, 
F. Dupertuis, 
P. Durante, 
R. Dzhelyadin, 
A. Dziurda, 
A. Dzyuba, 
S. Easo, 
U. Egede, 
V. Egorychev, 
S. Eidelman, 
D. van Eijk, 
S. Eisenhardt, 
U. Eitschberger, 
R. Ekelhof, 
L. Eklund, 
I. El Rifai, 
Ch. Elsasser, 
A. Falabella, 
C. F\"{a}rber, 
C. Farinelli, 
S. Farry, 
D. Ferguson, 
V. Fernandez Albor, 
F. Ferreira Rodrigues, 
M. Ferro-Luzzi, 
S. Filippov, 
M. Fiore, 
M. Fiorini, 
C. Fitzpatrick, 
M. Fontana, 
F. Fontanelli, 
R. Forty, 
O. Francisco, 
M. Frank, 
C. Frei, 
M. Frosini, 
E. Furfaro, 
A. Gallas Torreira, 
D. Galli, 
M. Gandelman, 
P. Gandini, 
Y. Gao, 
J. Garofoli, 
P. Garosi, 
J. Garra Tico, 
L. Garrido, 
C. Gaspar, 
R. Gauld, 
E. Gersabeck, 
M. Gersabeck, 
T. Gershon, 
Ph. Ghez, 
A. Gianelle, 
V. Gibson, 
L. Giubega, 
V.V. Gligorov, 
C. G\"{o}bel, 
D. Golubkov, 
A. Golutvin, 
A. Gomes, 
H. Gordon, 
M. Grabalosa G\'{a}ndara, 
R. Graciani Diaz, 
L.A. Granado Cardoso, 
E. Graug\'{e}s, 
G. Graziani, 
A. Grecu, 
E. Greening, 
S. Gregson, 
P. Griffith, 
L. Grillo, 
O. Gr\"{u}nberg, 
B. Gui, 
E. Gushchin, 
Yu. Guz, 
T. Gys, 
C. Hadjivasiliou, 
G. Haefeli, 
C. Haen, 
T.W. Hafkenscheid, 
S.C. Haines, 
S. Hall, 
B. Hamilton, 
T. Hampson, 
S. Hansmann-Menzemer, 
N. Harnew, 
S.T. Harnew, 
J. Harrison, 
T. Hartmann, 
J. He, 
T. Head, 
V. Heijne, 
K. Hennessy, 
P. Henrard, 
J.A. Hernando Morata, 
E. van Herwijnen, 
M. He\ss, 
A. Hicheur, 
D. Hill, 
M. Hoballah, 
C. Hombach, 
W. Hulsbergen, 
P. Hunt, 
T. Huse, 
N. Hussain, 
D. Hutchcroft, 
D. Hynds, 
V. Iakovenko, 
M. Idzik, 
P. Ilten, 
R. Jacobsson, 
A. Jaeger, 
E. Jans, 
P. Jaton, 
A. Jawahery, 
F. Jing, 
M. John, 
D. Johnson, 
C.R. Jones, 
C. Joram, 
B. Jost, 
N. Jurik, 
M. Kaballo, 
S. Kandybei, 
W. Kanso, 
M. Karacson, 
T.M. Karbach, 
I.R. Kenyon, 
T. Ketel, 
B. Khanji, 
S. Klaver, 
O. Kochebina, 
I. Komarov, 
R.F. Koopman, 
P. Koppenburg, 
M. Korolev, 
A. Kozlinskiy, 
L. Kravchuk, 
K. Kreplin, 
M. Kreps, 
G. Krocker, 
P. Krokovny, 
F. Kruse, 
M. Kucharczyk, 
V. Kudryavtsev, 
K. Kurek, 
T. Kvaratskheliya, 
V.N. La Thi, 
D. Lacarrere, 
G. Lafferty, 
A. Lai, 
D. Lambert, 
R.W. Lambert, 
E. Lanciotti, 
G. Lanfranchi, 
C. Langenbruch, 
T. Latham, 
C. Lazzeroni, 
R. Le Gac, 
J. van Leerdam, 
J.-P. Lees, 
R. Lef\`{e}vre, 
A. Leflat, 
J. Lefran\c{c}ois, 
S. Leo, 
O. Leroy, 
T. Lesiak, 
B. Leverington, 
Y. Li, 
M. Liles, 
R. Lindner, 
C. Linn, 
F. Lionetto, 
B. Liu, 
G. Liu, 
S. Lohn, 
I. Longstaff, 
J.H. Lopes, 
N. Lopez-March, 
P. Lowdon, 
H. Lu, 
D. Lucchesi, 
J. Luisier, 
H. Luo, 
E. Luppi, 
O. Lupton, 
F. Machefert, 
I.V. Machikhiliyan, 
F. Maciuc, 
O. Maev, 
S. Malde, 
G. Manca, 
G. Mancinelli, 
M. Manzali, 
J. Maratas, 
U. Marconi, 
P. Marino, 
R. M\"{a}rki, 
J. Marks, 
G. Martellotti, 
A. Martens, 
A. Mart\'{i}n S\'{a}nchez, 
M. Martinelli, 
D. Martinez Santos, 
D. Martins Tostes, 
A. Massafferri, 
R. Matev, 
Z. Mathe, 
C. Matteuzzi, 
A. Mazurov, 
M. McCann, 
J. McCarthy, 
A. McNab, 
R. McNulty, 
B. McSkelly, 
B. Meadows, 
F. Meier, 
M. Meissner, 
M. Merk, 
D.A. Milanes, 
M.-N. Minard, 
J. Molina Rodriguez, 
S. Monteil, 
D. Moran, 
M. Morandin, 
P. Morawski, 
A. Mord\`{a}, 
M.J. Morello, 
R. Mountain, 
I. Mous, 
F. Muheim, 
K. M\"{u}ller, 
R. Muresan, 
B. Muryn, 
B. Muster, 
P. Naik, 
T. Nakada, 
R. Nandakumar, 
I. Nasteva, 
M. Needham, 
S. Neubert, 
N. Neufeld, 
A.D. Nguyen, 
T.D. Nguyen, 
C. Nguyen-Mau, 
M. Nicol, 
V. Niess, 
R. Niet, 
N. Nikitin, 
T. Nikodem, 
A. Novoselov, 
A. Oblakowska-Mucha, 
V. Obraztsov, 
S. Oggero, 
S. Ogilvy, 
O. Okhrimenko, 
R. Oldeman, 
G. Onderwater, 
M. Orlandea, 
J.M. Otalora Goicochea, 
P. Owen, 
A. Oyanguren, 
B.K. Pal, 
A. Palano, 
M. Palutan, 
J. Panman, 
A. Papanestis, 
M. Pappagallo, 
L. Pappalardo, 
C. Parkes, 
C.J. Parkinson, 
G. Passaleva, 
G.D. Patel, 
M. Patel, 
C. Patrignani, 
C. Pavel-Nicorescu, 
A. Pazos Alvarez, 
A. Pearce, 
A. Pellegrino, 
G. Penso, 
M. Pepe Altarelli, 
S. Perazzini, 
E. Perez Trigo, 
P. Perret, 
M. Perrin-Terrin, 
L. Pescatore, 
E. Pesen, 
G. Pessina, 
K. Petridis, 
A. Petrolini, 
E. Picatoste Olloqui, 
B. Pietrzyk, 
T. Pila\v{r}, 
D. Pinci, 
A. Pistone, 
S. Playfer, 
M. Plo Casasus, 
F. Polci, 
G. Polok, 
A. Poluektov, 
E. Polycarpo, 
A. Popov, 
D. Popov, 
B. Popovici, 
C. Potterat, 
A. Powell, 
J. Prisciandaro, 
A. Pritchard, 
C. Prouve, 
V. Pugatch, 
A. Puig Navarro, 
G. Punzi, 
W. Qian, 
B. Rachwal, 
J.H. Rademacker, 
B. Rakotomiaramanana, 
M. Rama, 
M.S. Rangel, 
I. Raniuk, 
N. Rauschmayr, 
G. Raven, 
S. Redford, 
S. Reichert, 
M.M. Reid, 
A.C. dos Reis, 
S. Ricciardi, 
A. Richards, 
K. Rinnert, 
V. Rives Molina, 
D.A. Roa Romero, 
P. Robbe, 
D.A. Roberts, 
A.B. Rodrigues, 
E. Rodrigues, 
P. Rodriguez Perez, 
S. Roiser, 
V. Romanovsky, 
A. Romero Vidal, 
M. Rotondo, 
J. Rouvinet, 
T. Ruf, 
F. Ruffini, 
H. Ruiz, 
P. Ruiz Valls, 
G. Sabatino, 
J.J. Saborido Silva, 
N. Sagidova, 
P. Sail, 
B. Saitta, 
V. Salustino Guimaraes, 
B. Sanmartin Sedes, 
R. Santacesaria, 
C. Santamarina Rios, 
E. Santovetti, 
M. Sapunov, 
A. Sarti, 
C. Satriano, 
A. Satta, 
M. Savrie, 
D. Savrina, 
M. Schiller, 
H. Schindler, 
M. Schlupp, 
M. Schmelling, 
B. Schmidt, 
O. Schneider, 
A. Schopper, 
M.-H. Schune, 
R. Schwemmer, 
B. Sciascia, 
A. Sciubba, 
M. Seco, 
A. Semennikov, 
K. Senderowska, 
I. Sepp, 
N. Serra, 
J. Serrano, 
P. Seyfert, 
M. Shapkin, 
I. Shapoval, 
Y. Shcheglov, 
T. Shears, 
L. Shekhtman, 
O. Shevchenko, 
V. Shevchenko, 
A. Shires, 
R. Silva Coutinho, 
G. Simi, 
M. Sirendi, 
N. Skidmore, 
T. Skwarnicki, 
N.A. Smith, 
E. Smith, 
E. Smith, 
J. Smith, 
M. Smith, 
H. Snoek, 
M.D. Sokoloff, 
F.J.P. Soler, 
F. Soomro, 
D. Souza, 
B. Souza De Paula, 
B. Spaan, 
A. Sparkes, 
P. Spradlin, 
F. Stagni, 
S. Stahl, 
O. Steinkamp, 
S. Stevenson, 
S. Stoica, 
S. Stone, 
B. Storaci, 
S. Stracka, 
M. Straticiuc, 
U. Straumann, 
R. Stroili, 
V.K. Subbiah, 
L. Sun, 
W. Sutcliffe, 
S. Swientek, 
V. Syropoulos, 
M. Szczekowski, 
P. Szczypka, 
D. Szilard, 
T. Szumlak, 
S. T'Jampens, 
M. Teklishyn, 
G. Tellarini, 
E. Teodorescu, 
F. Teubert, 
C. Thomas, 
E. Thomas, 
J. van Tilburg, 
V. Tisserand, 
M. Tobin, 
S. Tolk, 
L. Tomassetti, 
D. Tonelli, 
S. Topp-Joergensen, 
N. Torr, 
E. Tournefier, 
S. Tourneur, 
M.T. Tran, 
M. Tresch, 
A. Tsaregorodtsev, 
P. Tsopelas, 
N. Tuning, 
M. Ubeda Garcia, 
A. Ukleja, 
A. Ustyuzhanin, 
U. Uwer, 
V. Vagnoni, 
G. Valenti, 
A. Vallier, 
R. Vazquez Gomez, 
P. Vazquez Regueiro, 
C. V\'{a}zquez Sierra, 
S. Vecchi, 
J.J. Velthuis, 
M. Veltri, 
G. Veneziano, 
M. Vesterinen, 
B. Viaud, 
D. Vieira, 
X. Vilasis-Cardona, 
A. Vollhardt, 
D. Volyanskyy, 
D. Voong, 
A. Vorobyev, 
V. Vorobyev, 
C. Vo\ss, 
H. Voss, 
J.A. de Vries, 
R. Waldi, 
C. Wallace, 
R. Wallace, 
S. Wandernoth, 
J. Wang, 
D.R. Ward, 
N.K. Watson, 
A.D. Webber, 
D. Websdale, 
M. Whitehead, 
J. Wicht, 
J. Wiechczynski, 
D. Wiedner, 
L. Wiggers, 
G. Wilkinson, 
M.P. Williams, 
M. Williams, 
F.F. Wilson, 
J. Wimberley, 
J. Wishahi, 
W. Wislicki, 
M. Witek, 
G. Wormser, 
S.A. Wotton, 
S. Wright, 
S. Wu, 
K. Wyllie, 
Y. Xie, 
Z. Xing, 
Z. Yang, 
X. Yuan, 
O. Yushchenko, 
M. Zangoli, 
M. Zavertyaev, 
F. Zhang, 
L. Zhang, 
W.C. Zhang, 
Y. Zhang, 
A. Zhelezov, 
A. Zhokhov, 
L. Zhong, 
A. Zvyagin


==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 18784 2012-04-30 14:45:53Z uegede $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}

